A Novel Information-Theoretic Objective to Disentangle Representations for Fair Classification

One of the pursued objectives of deep learning is to provide tools that learn abstract representations of reality from the observation of multiple contextual situations. More precisely, one wishes to extract disentangled representations which are (i) low dimensional and (ii) whose components are independent and correspond to concepts capturing the essence of the objects under consideration (Locatello et al., 2019b). One step towards this ambitious project consists in learning disentangled representations with respect to a predefined (sensitive) attribute, e.g., the gender or age of the writer. Perhaps one of the main application for such disentangled representations is fair classification. Existing methods extract the last layer of a neural network trained with a loss that is composed of a cross-entropy objective and a disentanglement regularizer. In this work, we adopt an information-theoretic view of this problem which motivates a novel family of regularizers that minimizes the mutual information between the latent representation and the sensitive attribute conditional to the target. The resulting set of losses, called CLINIC, is parameter free and thus, it is easier and faster to train. CLINIC losses are studied through extensive numerical experiments by training over 2k neural networks. We demonstrate that our methods offer a better disentanglement/accuracy trade-off than previous techniques, and generalize better than training with cross-entropy loss solely provided that the disentanglement task is not too constraining.

==> rebutal_1.tex <==


\section{First version}

\subsection{R1} 

The definition of disentangle and the some terms should be better described, or at least give comparison with other works.
The novelty of this paper is questionable, there are many papers work on contrastive learning, mutual information applied on different tasks. The contributions need more clarification.
Several experiments of other works should be added as compared baselines. The authors are encouraged to revise accordingly to above comments.

Weaknesses:

The definition of "disentanglement" in the paper is out of the mainstream of previous disentangled representation work. Disentangled representation is commonly defined among or between different parts of the latent representations[1,2,3,4]. However, the author defined the concept of "disengagement" as to reduce the correlation between latent representations and sensitive attributes, which to me is more like fair representation learning or representation debiasing.
The novelty of the method seems marginal. The learning objective in equation 3 is commonly used for unbiased representation learning [5,6], which is also motivated by the information-bottleneck methods. The proposed objective in equations 4 and 5 is also widely used in contrastive learning methods, which is a variant of the InfoNCE mutual information estimator.
The empirical results didn't compare with other disentanglement baseline methods, which is understandable because of the definition difference of "disentanglement".
[1] Understanding disentangling in β-VAE, NeurIPS 2017 [2] Challenging Common Assumptions in the Unsupervised Learning of Disentangled Representations, ICML 2019 [3] Disentangled Representation Learning for Non-Parallel Text Style Transfer, AAAI 2019 [4] Improving Disentangled Text Representation Learning with Information-Theoretic Guidance, ACL 2020 [5] FairFil: Contrastive Neural Debiasing Method for Pretrained Text Encoders, ICLR 2021 [6] Learning Unbiased Representations via Mutual Information Backpropagation, CVPR 2021

\subsection{R2} 
Weaknesses:
Assuming binary attributes being given a priori, which is not the case for most of the downstream tasks.
The phrase “mutual information maximization” in the title is rather misleading. This approach proposed in this paper does not explicitly involve a mutual information maximization objective.
I don’t see a clear connection between the components of Section 3: why does the motivation lead to a contrastive learning-based regularizer? I don’t follow Section 3.3, particularly Eq. 6 as to how the contrastive loss has to do with learning disentangled representations.

\subsection{R3} 
Weaknesses:
The evaluation on NLP insights are weak. Most of the results are measured by Y and S, which are metrics for disentangled representations. However, these intermediate metrics are NOT convincing from a practical point of view. How would improving the metrics of Y and S would impact a the real and important application metrics? For example, better classification accuracy in well established benchmarks? or better style transfer or controllable language generation? I would strongly suggest the authors study more useful downstream tasks to evaluate the methods to attract the attention of a broader audience, and thus achieve higher impact.
The current form of this paper is more like a general machine learning paper, which are evaluated by intermediate metrics only, and are potentially applicable to both NLP and CV etc. Though most of the experiments are done in NLP by adapting BERT or RNN encoders, the paper does not show fully convincing results. I am wondering, is there any related work closely related works, if the paper is positioned as a general machine learning paper.
Weaknesses:
The overall contribution seems incremental if considering the existence work in contrastive learning and mutual information maximization, such as InfoNCE. The main contribution that differentiate previous work is the sampling strategy.
In Table 2, as to the two columns "Y", it seems not the best models are highlighted as bold numbers.
\fi

